Exploring Camera Encoder Designs for Autonomous Driving Perception

The cornerstone of autonomous vehicles (AV) is a solid perception system, where camera encoders play a crucial role. Existing works usually leverage pre-trained Convolutional Neural Networks (CNN) or Vision Transformers (ViTs) designed for general vision tasks, such as image classification, segmentation, and 2D detection. Although those well-known architectures have achieved state-of-the-art accuracy in AV-related tasks, e.g., 3D Object Detection, there remains significant potential for improvement in network design due to the nuanced complexities of industrial-level AV dataset. Moreover, existing public AV benchmarks usually contain insufficient data, which might lead to inaccurate evaluation of those architectures.To reveal the AV-specific model insights, we start from a standard general-purpose encoder, ConvNeXt and progressively transform the design. We adjust different design parameters including width and depth of the model, stage compute ratio, attention mechanisms, and input resolution, supported by systematic analysis to each modifications. This customization yields an architecture optimized for AV camera encoder achieving 8.79% mAP improvement over the baseline. We believe our effort could become a sweet cookbook of image encoders for AV and pave the way to the next-level drive system.

==> experiments.tex <==
\section{Experiments}
\label{sect:experiments}


==> method.tex <==
% \section{Efficient perception models for Autonomous Driving}
% \label{sect:method}
% In this section, we first formulate the pruning process as an optimization process, before diving deep into the importance estimation for accuracy and latency. Then, we elaborate on how to solve the optimization via knapsack regime, augmented by dynamic grouping of neurons. We finalize the method by combining these key steps under one realm of HALP.

% \subsection{Objective Function}
% \label{sec:objective}
% Consider a neural network that consists of $L$ layers performing linear operations on their inputs, together with non-linear activation layers and potentially pooling layers. Suppose there are $N_{l}$ neurons (output channels) in the $l_{\text{th}}$ layer and each neuron is encoded by parameters $\textbf{W}_l^n\in \mathbb{R}^{C_l^{in}\times K_l \times K_l}$, where $C^{in}$ is the number of input channels and $K$ is the kernel size. By putting all the neurons across the network together, we get the neuron parameter set $\textbf{W}= \{\{\textbf{W}_l^n\}_{n=1}^{N_l}\}_{l=1}^L$, where $N=\sum_{l=1}^L N_l$ is the total number of neurons in the network. 

% Given a training set $\mathcal{D}=\{(x_i, y_i)\}_{i=1}^M$, the problem of network pruning with a given constraint $C$ can be generally formulated as the following optimization problem:
% \begin{equation}
% \small
%     \argmin_{\hat{\textbf{W}}}\mathcal{L}(\hat{\textbf{W}}, \mathcal{D}) 
%     \quad \text{s.t.} \quad \Phi\left(f(\hat{\textbf{W}}, x_i)\right) \leq {C}
% \end{equation}
% \noindent
% where $\hat{\textbf{W}} \subset \textbf{W}$ is the remaining parameters after pruning and $\mathcal{L}$ is the loss of the task. $f(\cdot)$ encodes the network function, and $\Phi(\cdot)$ maps the network to the constraint $C$, such as latency, FLOPs, or memory. We primarily focus on latency in this work while the method easily scales to other constraints.

% The key to solving the aforementioned problem relies on identifying the portion of the network that satisfies the constraint while incurring minimum performance disruption:
% \begin{equation}
% \label{problem_formulatets}
% \small
%     \begin{split}
%     \argmax_{p_1, \cdots, p_l}\sum_{l=1}^L I_l(p_l), 
%     \ \text{s.t.} \
%     \sum_{l=1}^{L} T_l(p_{l-1}, p_l) \leq C, \ \forall l \ \ 0\leq p_l \leq N_l
%     \end{split}
% \end{equation}
% \noindent
% where $p_l$ denotes the number of kept neurons at layer $l$, $I_l(p_l)$ signals the maximum importance to the final accuracy with $p_l$ neurons, and $T_l(p_{l-1}, p_l)$ checks on the associated latency contribution of layer $l$ with $p_{l-1}$ input channels and $p_l$ output channels. $p_0$ denotes a fixed input channel number for the first convolutional block, \eg, $3$ for RGB images. 
% We next elaborate on $I(\cdot)$ and $T(\cdot)$ in detail.

% \textbf{Importance score.} To get the importance score of a layer to final accuracy, namely $I_l(p_l)$ in Eq.~\ref{problem_formulatets}, we take it as the accumulated score from individual neurons $\sum_{j=1}^{p_l}\mathcal{I}_l^j$. We first approximate the importance of neurons using the Taylor expansion of the loss change~\cite{molchanov2019importance}. 
% Specifically, we prune on batch normalization layers and the importance of the $n$-th neuron in the $l$-th layer is calculated as
% \begin{equation}
% \label{importance_calc}
%     \mathcal{I}_l^n = \left|g_{\gamma_l^n}\gamma_l^n+g_{\beta_l^n}\beta_l^n \right|,
% \end{equation}
% where $g$ denotes the gradient of the weight, $\gamma_l^n$ and $\beta_l^n$ are the corresponding weight and bias from the batch normalization layer, respectively. Unlike a squared loss in~\cite{molchanov2019importance}, we use absolute difference as we observe slight improvements.

% In order to maximize the total importance, we keep the most important neurons at a higher priority. 
% To this end, we rank the neurons in the $l_{th}$ layer according to their importance score in a descending order and denote the importance score of the $j_{th}$-ranked neuron as $\mathcal{I}_l^j$, thus we have
% \begin{equation}
% \label{layer_importance}
% \small
%     I_l(p_l) = \sum_{j=1}^{p_l}\mathcal{I}_l^j, 
%     \quad  
%     0 \leq p_l \leq N_l, \
%     \mathcal{I}_l^1 \geq \dots \geq \mathcal{I}_l^{N_l}.
% \end{equation}
% \textbf{Latency contribution.} We empirically obtain the layer latency $T_l(p_{l-1}, p_l)$ in Eq.~\ref{problem_formulatets} by pre-building a layer-wise look-up table with pre-measured latencies. This layer latency corresponds to the aggregation of the neuron latency contribution of each neuron in the layer, $c_l^j$:
% \begin{equation}
% \label{layer_latency}
% \small
%     \quad T_l(p_{l-1}, p_l) = \sum_{j=1}^{p_l}c_l^j,
%     \quad 
%     0 \leq p_l \leq N_l. \
% \end{equation}
% The latency contribution of the $j$-th neuron in the $l$-th layer can also be computed using the entries in the look up table as:
% \begin{equation}
% \label{latency_calculate}
% \small
%     c_l^j = T_l{(p_{l-1}, j)} - T_l{(p_{l-1}, j-1)}, \quad 1 \leq j \leq p_l.
% \end{equation}

% In practice, we first rank globally neurons by importance and then consider their latency contribution. Thus, we can draw the following properties. If we remove the least important neuron in layer $l$, then the number of neurons will change from $p_l$ to $p_l-1$, leading to a latency reduction $c_l^{p_l}$ as this neuron's latency contribution score. 
% We assign the potential latency reduction to neurons in the layer by the importance order. The most important neuron in that layer would always have a latency contribution $c_l^1$.
% At this stage, finding the right combination of neurons to keep imposes a combinatorial problem, and in the next section we tackle it via reward maximization considering latency and accuracy traits. 





% \subsection{Augmented Knapsack Solver} 
% \label{sec:solver}
% Given both importance and latency estimates, we now aim at solving Eq.~\ref{problem_formulatets}. By plugging back in the layer importance Eq.~\ref{layer_importance} and layer latency Eq.~\ref{layer_latency}, we come to
% \begin{equation}
% \small
%     \label{modified_optimization}
%     \max\sum_{l=1}^L\sum_{j=1}^{p_l} \mathcal{I}_l^j, 
%     \quad \text{s.t.} \quad
%     \sum_{l=1}^{L}\sum_{j=1}^{p_l} c_l^j \leq C, \quad 0\leq p_l \leq N_l, \quad
%     \mathcal{I}_l^1 \geq \mathcal{I}_l^2 \geq \dots \mathcal{I}_l^{N_l}.
% \end{equation} 
% \noindent
% This simplifies the overall pruning process into a knapsack problem only with additional preceding constraints. The preceding enforcement originates from the fact that for a neuron with rank $j$ in the $l_{th}$ layer, the neuron latency contribution only holds when all the neurons with rank $r=1,\dots,j-1$ are kept in the $l_{th}$ layer and the rest of the neurons with rank $r = j+1, j+2, \cdots, N_l$ are removed. Yet the problem is solvable by specifying each item with a list of preceding items that need to be selected before its inclusion. 

% We augment the knapsack solver to consider the reordered neurons with descending importance score so that all the preceding neurons will be processed before it. A description of the pseudo code of the augmented knapsack solver is provided in Algo.~\ref{modified-knapsack-solution} (a detailed explanation is provided in Appendix~\ref{algo_explain}). The augmented solver is required to make sure that the latency cost is correct.
% \begin{algorithm}[!t]
%      \tiny
%     \caption{Augmented Knapsack Solver}
%     \label{modified-knapsack-solution}
%     \textbf{Input:} Importance score $\{\mathcal{I}_l \in \mathbb{R}^{N_l}\}_{l=1}^L$ where $\mathcal{I}_l$ is sorted descendingly; Neuron latency contribution $\{c_l\in \mathbb{R}^{N_l} \}_{l=1}^L$; Latency constraint $C$.
%     \begin{algorithmic}[1]
%         \State $\text{maxV} \in \mathbb{R}^{(C+1)}$, $\text{keep} \in \mathbb{R}^{L\times (C+1)}$ \Comment{maxV[$c$]: max importance under constraint $c$; keep[$l$, $c$]: \# neurons to keep in layer $l$ to achieve maxI[$c$]}
%         \For{$l = 1, \dots, L$}
%         \For{$j = 1, \dots, N_l$}
%             \For{$c = 1, \dots, C$}
%                 \State $v_{\text{keep}} = \mathcal{I}_l^j + \text{maxV}[c - c_l^j]$, \ $v_{\text{prune}} = \text{maxV}[c]$ \Comment{total importance can achieve under constraint $c$ with object $n$ being kept or not}
%                 \If{$v_{\text{keep}} > v_{\text{prune}}$ \textbf{and} $\text{keep}[l, c-c_l^j] == j-1$} \Comment{check if it leads to higher score and if more important neurons in layer are kept}
%                     \State $\text{keep}[l, c] = j$, \ $\text{update\_maxV}[c]=v_{\text{keep}}$
%                 \Else 
%                     \State $\text{keep}[l, c] = \text{keep}[l, c-1]$, \ $\text{update\_maxV}[c]=v_{\text{prune}}$
%                 \EndIf
%             \EndFor
%             \State $\text{maxV} \leftarrow \text{update\_maxV}$
%         \EndFor
%         \EndFor \\
        
%         \State $\text{keep\_n} = \O$ to save the kept neurons in model
        
%         \For{$l = L, \dots, 1$}  \Comment{retrieve the set of kept neurons}
%             \State $p_l = \text{keep}[l, C]$ 
%             \State $\text{keep\_n} 
%             \leftarrow \text{keep\_n} \cup \{p_l \ \text{top ranked neurons in layer} \ l\}$
%             \State $C 
%             \leftarrow C - \sum_{j=1}^{p_l}c_l^j$
%         \EndFor
%     \end{algorithmic}
%     \textbf{Output:} Kept important neurons ($\text{keep\_n}$).
% \end{algorithm}


% % \subsection{Neuron Grouping}
% % \label{neuron-grouping}
% % Considering each neuron individually results in burdensome computation during pruning. We next explore grouping neurons so that a number of them can be jointly considered and removed enabling faster pruning~\cite{yin2020dreaming}. Neuron grouping helps exploit hardware-incurred channel granularity guided by the latency, speeds up knapsack solving of Eq.~\ref{modified_optimization}, and yields structures that maximize the GPU utilization, keeping as many parameters as possible under the similar latency. In addition, neuron grouping simplifies the knapsack problem that scales linearly with the number of candidates under consideration (see Line $3$ of Alg.~\ref{modified-knapsack-solution}), thus speedups the solver as we'll discuss later.


% % %This helps exploit hardware-incurred channel granularity guided by the latency, and speed up knapsack solving of Eq.~\ref{modified_optimization}. In addition, neuron grouping simplifies the knapsack problem that scales linearly with the number of candidates under consideration (see Line $3$ of Alg.~\ref{modified-knapsack-solution}), thus speedups the solver as we'll discuss later. It also helps fully exploit the latency landscape and yields structures that maximize the GPU utilization, keeping as many parameters as possible under the similar latency.



% % We refer to the difference of neuron counts between two latency cliffs of the staircase-patterned latency as the latency step size.
% % In our method, we group $s$ channels in a layer as an entirety, where the value of $s$ is equal to the latency step size. The neurons are grouped by the order of importance. Then we aggregate the importance score and latency contribution for the grouped entity.
% % For skip connections in ResNet and group convolutions in MobileNet, we not only group neurons within a layer, we also group the neurons sharing the same channel index from the connected layers~\cite{ding2019centripetal, luo2020neural}. For cross-layer grouping, as the latency step size for different layers might be different, we use the largest group size among the layers. 
% % Latency-aware grouping enables additional performance benefits when compared to a heuristic universal grouping, as we will later show in the experiments.

% % %One noticeable benefit of neuron grouping is the simplification of knapsack problem that scales linearly with the number of candidates under consideration (see Line $3$ of Alg.~\ref{modified-knapsack-solution}), which speedups the solver as we'll discuss later. It also helps fully exploit the latency landscape and yields structures that maximize the GPU utilization, keeping as many parameters as possible under the similar latency.
% % % As an example, by grouping neurons for a ResNet50, the total number of (grouped) neurons can be greatly reduced from $26,560$ to only $215$, this drastically speedups the solver. Such saving can be especially beneficial as network size scales up, a very likely trend that literature foresees. 

% \subsection{Final HALP Regime} 
% With all aforementioned steps, we formulate the final HALP as follows. The pruning process takes a trained network as input and prunes it iteratively to satisfy the requirement of a given latency budget $C$. We perform one pruning every $r$ minibatches and repeat it $k$ pruning steps in total. In particular, we set $k$ milestones gradually decreasing the total latency to reach the goal via exponential scheduler~\cite{de2020force}, with $C^1 > C^2 > \cdots > C^k$, $C^k=C$. The algorithm gradually trims down neurons using steps below:
% \begin{itemize}[topsep=1pt,itemsep=1pt,partopsep=0pt, parsep=0pt,leftmargin=\labelwidth]
%     \item \textbf{Step 1}. For each minibatch, we get the gradients of the weights and update the weights as during the normal training. We also calculate each neuron's importance score as Eq.~\ref{importance_calc}. 
%     \item \textbf{Step 2}. Over multiple minibatches we calculate the average importance score for each neuron  and rank them accordingly. Then we count the number of neurons remaining in each layer and dynamically adjust the latency contribution as in Eq.~\ref{latency_calculate}.
%     \item \textbf{Step 3}. We group neurons as described in Sec.~\ref{neuron-grouping} and calculate group's importance and latency reduction. Then we get the nearest preceding group for each layer.
%     \item \textbf{Step 4}. We execute the Algo.~\ref{modified-knapsack-solution} to select the neurons being remained with current latency milestone. Repeat starting from the Step 1 until $k$ milestones are reached.
% \end{itemize}
% Once pruning finishes we fine-tune the network to recover accuracy.



==> random.tex <==

Why Training as a post-processing:
- Simpler
- Shown good results despite some benefits in training costs shown in Shen CVPR
- Dense larger model can be used for offline tasks such as autolabeling and future - distillation to reduce accuracy drop



Why AlexNet v2 -> train compromise and then light prune
-- Show results for expanded models - and the benefit of training and then compress. 
-- Do we need shorter training time?

-- What happens when we care about the training cost / simplicity
-- Basically, not only the cost, but the simplicity of operations and traceability in the infrastructure. 



 --- Conclusions
 Train large then compress provides a better trade-off and reusability of the models. Easier to converge and more prunable -- aka, less accuracy drop when pruned. This is particularly true for large scale experiments (datasets) when there is no overfitting issues. In small scale, large models can be pruned very aggressively without accuracy drops. 

 Under that assumption, current pruning methods tend to focus on light / medium compression rates, and therefore, fail to compress for extreme ratios. That is work in progress~\cite{Ryan}
 
 In those settings, it is also important to consider the cost of training and the trade off for latency-accuracy. Our experiments suggest that training extremely large models might not be beneficial if those larger models can not be reused for other "offline" tasks, as they require easily 40\% additional training cost while not bringing any performance benefits. 

 








3D object detection is vital as it would enable us to capture objects' sizes, orientation, and position in the world.


To obtain a comprehensive understanding of driving environments, many vision tasks can be involved in a perception system, e.g. object detection and tracking, lane detection, semantic and instance segmentation, etc. Among these perception tasks, 3D object detection is one of the most indispensable tasks in an automotive perception system. 3D object detection aims to predict the locations, sizes, and classes of critical objects, e.g. cars, pedestrians, cyclists, etc., in the 3D space. In contrast to object detection that only generates 2D bounding boxes on images and ignores the actual distance information of objects from the ego-vehicle, 3D object detection focuses on the localization and recognition of objects in the real-world 3D coordinate system. The geometric information predicted by 3D object detection in real-world coordinates can be directly utilized to measure the distances between the ego-vehicle and critical objects, and to further help plan driving routes and avoid collisions.


Vision based 3D object detection




3D methods have to consider different views to detect 3D objects, e.g. from the bird’s-eye view, point view, cylindrical view, etc. (3) 3D object detection has a high demand for accurate localization of objects in the 3D space.





It is because the rapid growth of the model size that model optimization techniques become a particularly relevant area of study. 

For industry, as the training resources are costly and limited, there is a need to adopt compute-efficient training strategies. For this reason, 

For self-driving, as for many other real-world problems, the cost of inference usually dominates the cost of training, and therefore, 


to scale to massive amounts of data and very large models. As a consequence, computational resources are increasingly the critical constraint to deploy this models. It is not only the increasing number of compute but also the longer training times required to produce deployable models. This causes industry to adopt training strategies that maximize compute efficiency: training strategies that, given a fixed amount of hardware and training time, yield the highest model accuracy under certain latency budget constraints. 

A common approach is to train a reasonably compact model that achieves good accuracy with a reasonably close forward time and then, apply light model optimization techniques such as network quantization to meet the required real-time constraints without compromising the accuracy. However, as we will show in this paper, this might lead to suboptimal performance as "compact" models are usually harder to train to convergence to achieve their maximum performance~\cite{}. In addition, these models are more sensitive to quantization and pruning as they tend to have lower flexibility and parameter redundancy. 

In contrast, large models tend to be easier to train, yield much higher accuracy and, in general, they are more robust to compression. However, as the models increase the size, so do the needs for increasing the compression ratios. In addition, these larger models yielding much higher performance can be also used for other tasks such as offline pseudolabeling or in teacher-student configurations for improving the accuracy of compact models~\cite{}.

In this paper, we analyze the benefits of neural network pruning for maximizing the latency-accuracy trade-off while maintaining the training cost under control. \textbf{for 3D object detection.} To that end, we analyze the benefits of training larger models and adopting heavier compression mechanisms like neural network pruning. In addition, we study the effect of the model size to this approach. 





Aggressively pruning large models is an option for simple tasks and small scale data when the model is clearly overparameterized. However, as the complexity of the task increases and so does the size of the dataset, the effectiveness of pruning aggressively a model decreases. For instance, there is a X\% accuracy drop when pruning 60\% a resnet50 for ImageNet. In contrast, pruning a resnet50 for 2D object detection in small dataset yields up to Xx latency speeds up without accuracy drops. See experiments on 2D object detection in TableXX. 




As we will see, this option greatly benefits the latency-accuracy trade-off while not incurring in prohibitive training costs. 









Therefore, the most compute-efficient training strategy is to counter intuitively train extremely large models but stop after a small number of iterations. T

Since hardware resources are limited, the objective of training deep learning models is typically to maximize accuracy subject to the time Common Practice Train Small Model Optimal Stop Training When Converged Train Large Model Lightly Compress Stop Training Early and memory constraints of training and inference




As systems evolve so do the compute needs to get those systems trained 


Deep learning and, in particular, end-to-end learning has enabled better and better perception models. However, this has generally come at the cost of exponentially increasing their size, and, as a consequence limiting their feasibility to be deployed for real time applications. These models not only need to meet real time constraints but also need to run in resource-limited platforms.

As a consequence, large scale models and data (and hence compute budgets) are paramount de facto for the attainment of high-performance.





However, in order to deploy these models, they need to meet real-time constraints in resource-limited platforms. 


While overparametrized large language models achieve state-of-the-art NLP performance, they raise concern about environmental impact, training cost, and feasibility of deployment in edge devices. Model compression promises to alleviate these issues, and multiple approaches have recently been successful in decreasing the number of parameters.



\section{Object detection for AV \& Multi-camera 3D object detection for AV}

As the number of cameras increases so does the compute needed during training and inference. 





The goal of simplifying the training pipeline by using specific architectures has the additional cost of needed to find the right archtiecture for the given hardware. In general, compact architectures are less explored in the literature and should be specific to the target device. A common approach to this is using neural architecture search (manual or algorithmic) or, in the best case scenario, instantiate pruning to perform at an early stage of training. However, neural architecture search requires a surprisingly large cost to find the right architecture and, in addition, it usually has a limited search space, therefore, might lead to suboptimal performance in the target hardware. The second, pruning at initialization has proved to be very effective, but in general, leads to slightly lower performance compared to pruning while training or pruning as a postprocessing step. In addition, for both cases, the trained model can not effectively used for offline tasks as its performance is the exact trade off between accuracy and latency. 


\section{Latency-aware Network Pruning}






\section{Multi-camera 3D object detection experiments}


\section{discussion}


 

% \section{Introduction}
% An important barrier in the deployment of deep neural networks is latency, which is critical for autonomous driving tasks. High latency can lead to delayed recognition of an object or a pedestrian in front of the car, making it challenging to take the appropriate maneuver in time. For this reason, practitioners have been forced to use shallow networks with non-ideal accuracy to avoid this latency problem. We plan to address this challenge by developing a systematic multi-faceted approach for end-to-end efficient NN design and deployment by pursuing the following thrusts: (i) developing a fast coupled quantization and pruning framework that allows the practitioner to obtain optimal trade-offs between accuracy, and speed for a given latency constraint; (ii) developing a quantization and pruning aware Neural Architecture Search co-designed for a target hardware platform for autonomous driving with limited power budget; and (iii) focusing on object detection and segmentation applications with 4K video stream. The outcome of this work will be an open-source framework that will automatically find an efficient NN architecture for the application-specific constraints of accuracy, latency, model size, and power consumption. This will build upon our recent works on quantization~\cite{dong2019hawq,dong2019hawqv2,yao2020hawqv3,cai2020zeroq}, pruning~\cite{yu2021hessian}, NAS~\cite{wu2018mixed,wu2019fbnet}, and the corresponding open source codes that have been contributed to BDD repository


% Deep neural networks have rapidly developed over the last decade and come to dominate many traditional algorithms in a wide range of tasks. In particular, convolutional neural networks (CNNs) have shown state-of-the-art results on a range of computer vision tasks, including classification, detection, and segmentation. However, modern CNNs have grown in size, computation, energy requirement, and prediction latency, as researchers push for accuracy improvements. Unfortunately, these models can now easily exceed the capabilities of many edge computing devices and requirements of real-time inference tasks, such as those found in autonomous vehicle applications.



% Since neural networks have been shown to be heavily over-parameterizered \cite{zhang_2017}, one popular method for reducing the computation and prediction latency is to prune (or remove) portions of the neural network, ultimately yielding a model with fewer parameters. Due to the strict requirements for many deployment applications, a large fraction of the parameters often must be removed; we focus on this regime, which we refer to as the high pruning ratio regime. Towards this aim, many pruning methods have been proposed to identify and remove those parameters that are least important for inference~\cite{alvarez_2016,he_2017_pruning,luo_2017,lecun_1989,molchanov_2019,ye_2018,yu_2018}. Since each layer of the network involves a different computation and associated computational burden, each parameter does not contribute equally to the final network inference cost, typically measured as FLOPs or latency, so more recent works have focused on pruning the network subject to explicit cost constraints. To maximize inference speedup on modern hardware (e.g., GPUs), these works largely focus on channel pruning~\cite{li_2020,luo_2017,molchanov_2019,shen_2021,wang_2021,yu_2019}.
% % \JM{maybe something regarding high pruning ratios for motivating}











% \begin{figure}[!t]
%   \centering
%   \resizebox{\columnwidth}{!}{
%   \includegraphics[width=1.0\linewidth]{images/MainResults.png}
%   }
%   \caption{Main Results.}
%   \label{fig:architecture}
%   \vspace{-0.5cm}
% \end{figure}

==> realtedwork.tex <==
\section{Related Work}
\label{sect:sota}



